Computational Distinguishability of Quantum Channels

The computational problem of distinguishing two quantum channels is central to quantum computing. It is a generalization of the well-known satisfiability problem from classical to quantum computation. This problem is shown to be surprisingly hard: it is complete for the class QIP of problems that have quantum interactive proof systems, which implies that it is hard for the class PSPACE of problems solvable by a classical computation in polynomial space. Several restrictions of distinguishability are also shown to be hard. It is no easier when restricted to quantum computations of logarithmic depth, to mixed-unitary channels, to degradable channels, or to antidegradable channels. These hardness results are demonstrated by finding reductions between these classes of quantum channels. These techniques have applications outside the distinguishability problem, as the construction for mixed-unitary channels is used to prove that the additivity problem for the classical capacity of quantum channels can be equivalently restricted to the mixed unitary channels.

==> figures/gate-S.latex <==
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(774,474)(4189,2)
\thinlines
{\color[rgb]{0,0,0}\put(4351, 14){\framebox(450,450){$S$}}
}%
{\color[rgb]{0,0,0}\put(4351,239){\line(-1, 0){150}}
}%
{\color[rgb]{0,0,0}\put(4801,239){\line( 1, 0){150}}
}%
\end{picture}%


==> figures/gate.latex <==
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(774,474)(4189,2)
\thinlines
{\color[rgb]{0,0,0}\put(4351, 14){\framebox(450,450){}}
}%
{\color[rgb]{0,0,0}\put(4351,239){\line(-1, 0){150}}
}%
{\color[rgb]{0,0,0}\put(4801,239){\line( 1, 0){150}}
}%
\end{picture}%


==> makefile <==
#
# Modified version of makefile found at:
# http://xpt.sourceforge.net/techdocs/Latex/MakefileForTeX/Latex08.000.html
#
# Author seems to be: Anthony Piron (apiron@brutele.be)
# In a post to comp.text.tex, dejanews link is:
# http://groups.google.com/groups?hl=en&lr=&ie=UTF-8&selm=3A9640D7.D6A40946%40brutele.be

LATEX = latex -interaction=nonstopmode
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = pdflatex -interaction=nonstopmode
DVIPS = dvips
MAKEINDEX = makeindex
TOUCH = touch
LS = ls
TEST = test

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right|No file *.[toc,aux,tof])"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "Writing index file .*\.idx"
MAKENCL = "Writing nomenclature file .*\.nlo"
TARGET = thesis

GOALS = 	$(TARGET).ps $(PDF)
PDF   = 	$(TARGET).pdf
DVIFILES = 	$(TARGET).dvi

main:	$(PDF)

final: 	empty main

all:	clean main

pdf:	$(TARGET).pdf

ps:		$(TARGET).ps

%.dvi:	%.tex
		$(LATEX) $<
		@egrep $(MAKEIDX) $*.log && ($(MAKEINDEX) $*;$(TOUCH) $*.flag) ; true
		@egrep $(MAKENCL) $*.log && ($(MAKEINDEX) $*.nlo -s nomencl.ist -o $*.nls;$(TOUCH) $*.flag) ; true
		@egrep $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(TOUCH) $*.flag) ; true
		@$(TEST) -f $*.flag && ($(LATEX) $<; rm $*.flag) ; true
		@egrep $(RERUN) $*.log && ($(LATEX) $<) ; true
		@egrep $(RERUN) $*.log && ($(LATEX) $<) ; true

# Display relevant warnings
		@egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:	%.dvi
		$(DVIPS) $< -o $@

%.pdf:	%.tex
		$(PDFLATEX) $<
		@egrep $(MAKEIDX) $*.log && ($(MAKEINDEX) $*;$(TOUCH) $*.flag) ; true
		@egrep $(MAKENCL) $*.log && ($(MAKEINDEX) $*.nlo -s nomencl.ist -o $*.nls;$(TOUCH) $*.flag) ; true
		@egrep $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(TOUCH) $*.flag) ; true
		@$(TEST) -f $*.flag && ($(PDFLATEX) $<; rm $*.flag) ; true
		@egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
		@egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true

# Display relevant warnings
		@egrep -i "(Reference|Citation).*undefined" $*.log ; true


clean:
		for i in $$( ls | grep '\.tex' | awk -F '.' '{print $$1}' ); \
			do rm -f $$i.aux; done
		rm -f $(TARGET).aux $(TARGET).bbl $(TARGET).blg \
	 	      $(TARGET).dvi $(TARGET).lof $(TARGET).log \
	 	      $(TARGET).idx $(TARGET).ilg $(TARGET).ind \
	 	      $(TARGET).nlo $(TARGET).nls $(TARGET).pdfsync \
	 	      $(TARGET).mtc* $(TARGET).maf \
				$(TARGET).lot $(TARGET).toc $(TARGET).out *~

empty: 	clean
		rm -f $(TARGET).pdf $(TARGET).ps

thesis.dvi: *.tex figures/*.latex  figures/*.epic
thesis.pdf: *.tex figures/*.latex  figures/*.epic

